Bibliometric Analysis of Scientific Publications on Blockchain Research and Applications

Since the introduction of Bitcoin in 2008, blockchain technology has garnered widespread attention. Scholars from various research fields, countries, and institutions have published a significant number of papers on this subject. However, there is currently a lack of comprehensive analysis specifically focusing on the scientific publications in the field of blockchain. To conduct a comprehensive analysis, we compiled a corpus of 41,497 publications in blockchain research from 2008 to 2023 using the Clarivate databases. Through bibliometric and citation analyses, we gained valuable insights into the field. Our study offers an overview of the blockchain research landscape, including country, institution, authorship, and subject categories. Additionally, we identified Emerging Research Areas (ERA) using the co-citation clustering approach, examining factors such as recency, growth, and contributions from different countries/regions. Furthermore, we identified influential publications based on citation velocity and analyzed five representative Research Fronts in detail. This analysis provides a fine-grained examination of specific areas within blockchain research. Our findings contribute to understanding evolving trends, emerging applications, and potential directions for future research in the multidisciplinary field of blockchain.

==> tables/table-5-1.tex <==
\begin{table*}[]
\centering
\caption{Metrics Calculated For Each Selected ERA}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lp{0.8\textwidth}@{}}
\toprule
\textbf{Name}                       & \textbf{Description}                                                                                                                                  \\ \midrule
Area                                  & Name of the Emerging Research Area (ERA)                                                                                                \\
% Name - Key terms                    & The list of key terms describing the ERA                                                                                                              \\
Size of foundation                  & The overall number of core papers. The number of core RF papers would range from 2 to 50 by original definition in the Research Front methodology     \\
% Number of co-citing papers          & The number of publications in the ERA co-citing the core Research Front papers                                                                        \\
% Number of all citing papers         & The number of all publications citing the core Research Front papers                                                                                  \\
Recency                             & The average publication year of core papers, this would indicate when the Research Front emerged                                                      \\
% Emergence                           & The average publication year of citing publications, this would indicate to what extent the research referencing the Research Front is contemporary   \\
Growth                              & The average annual growth rate of co-citing papers, this would measure how fast the Research Front is growing. Growth is not shown for recent ERAs.   \\
% Interdisciplinarity                 & The assessment of the degree to which the core papers are integrating knowledge from different fields using Porter’s integration index of core papers \\
% Country/Region contribution to Core & The number of Research Front core papers that have at least one affiliation in selected country/region                                                \\
Country/Region contribution to ERA  & The number of ERA publications (core + co-citing) that have at least one affiliation in selected country/region                                       \\
% ZJU contribution to Core            & The number of Research Front core papers that have at least one affiliation in ZJU                                                                    \\
% ZJU contribution to ERA             & The number of ERA publications (core + co-citing) that have at least one affiliation in ZJU                                                           \\
% Top ESI category                    & The most frequent ESI subject area within the ERA (core + co-citing)                                                                                  \\ 
\bottomrule
\end{tabular}
}
\label{tab:5-1}
\end{table*}
